MLPerf Inference Benchmark

Machine-learning (ML) hardware and software system demand is burgeoning. Driven by ML applications, the number of different ML inference systems has exploded. Over 100 organizations are building ML inference chips, and the systems that incorporate existing models span at least three orders of magnitude in power consumption and five orders of magnitude in performance; they range from embedded devices to data-center solutions. Fueling the hardware are a dozen or more software frameworks and libraries. The myriad combinations of ML hardware and ML software make assessing ML-system performance in an architecture-neutral, representative, and reproducible manner challenging. There is a clear need for industry-wide standard ML benchmarking and evaluation criteria. MLPerf Inference answers that call. In this paper, we present our benchmarking method for evaluating ML inference systems. Driven by more than 30 organizations as well as more than 200 ML engineers and practitioners, MLPerf prescribes a set of rules and best practices to ensure comparability across systems with wildly differing architectures. The first call for submissions garnered more than 600 reproducible inference-performance measurements from 14 organizations, representing over 30 systems that showcase a wide range of capabilities. The submissions attest to the benchmark's flexibility and adaptability.

==> table/performance_summary.tex <==
\begin{table}[b!] 
 \caption{Closed-division performance summary across tasks and scenarios. Each entry is the ratio of the highest to lowest performance. The performance range is as much as 10,000x. GNMT appears as N/A for multistream because it had no submissions.}
 \label{tab:performance}
    \vskip 0.05in
 \vskip 0.05in
  \begin{center}
 \begin{sc}
 \begin{adjustbox}{width=\columnwidth, center}
\begin{tabular}{c | c | c | c | c }
\toprule
 & \textbf{Single-Stream} & \textbf{Multistream} & \textbf{Server}  & \textbf{Offline} \\
\midrule
\textbf{GNMT} & 2 & N/A & 5 & 2,367 \\
\hline
\textbf{MobileNet-v1} & 1,199 & 29 & 9 & 438  \\
\hline
\textbf{ResNet-50v1.5} & 11154 & 27 & 26 & 10,289  \\
\hline
\textbf{SSD-MobileNet-v1} & 8 & 36 & 25 & 657 \\
\hline
\textbf{SSD-ResNet34} & 8 & 44 & 9 & 147 \\

\bottomrule
\end{tabular}
\end{adjustbox}
\end{sc}
\end{center}
\vskip -0.15in
\end{table}

==> tex/acks_long.tex <==
\section{Acknowledgements}
\label{sec:acks}

MLPerf Inference is the work of many individuals from multiple organizations. In this section, we acknowledge all those who helped produce the first set of results or supported the overall benchmark development. 

% \section*{Alibaba T-Head}

% Zhi Cai,
%  Danny Chen,
%  Liang Han,
%  Jimmy He,
%  David Mao,
%  Benjamin Shen,
%  ZhongWei Yao,
%  Kelly Yin,
%  XiaoTao Zai,
%  Xiaohui Zhao,
%  Jesse Zhou,
%  and
%  Guocai Zhu.

% \section*{Baidu}
% Newsha Ardalani, Ken Church, and Joel Hestness.

% \section*{Cadence}
% Debajyoti Pal.

% \section*{Centaur Technology}
% Bryce Arden,
%  Glenn Henry,
%  CJ Holthaus,
%  Kimble Houck,
%  Kyle O'Brien,
%  Parviz Palangpour,
%  Benjamin Seroussi,
%  and
%  Tyler Walker.

% \section*{Dell EMC}
% Frank Han, Bhavesh Patel, Vilmara Rocio Sanchez,  and
% Rengan Xu.

% \section*{dividiti}
% Grigori Fursin and Leo Gordon. 

% \section*{Facebook}
% Soumith Chintala, Kim Hazelwood, Bill Jia,  and
% Sean Lee.

% \section*{FuriosaAI}
% Dongsun Kim and Sol Kim.

% \section*{Google}
%  Michael Banfield,
%  Victor Bittorf,
%  Bo Chen,
%  Dehao Chen,
%  Ke Chen,
%  Chiachen Chou,
%  Sajid Dalvi,
%  Suyog Gupta,
%  Blake Hechtman,
%  Terry Heo,
%  Andrew Howard,
%  Sachin Joglekar,
%  Allan Knies,
%  Naveen Kumar,
%  Cindy Liu,
%  Thai Nguyen,
%  Tayo Oguntebi,
%  Yuechao Pan,
%  Mangpo Phothilimthana, 
%  Jue Wang,
%  Shibo Wang,
%  Tao Wang,
%  Qiumin Xu,
%  Cliff Young,
%  Ce Zheng, 
%  and
%  Zongwei Zhou.
 
% \section*{Hailo}
% Ohad Agami, Mark Grobman,  and
% Tamir Tapuhi.

% \section*{Intel}
% Md Faijul Amin,
%  Thomas Atta-fosu,
%  Haim Barad,
%  Barak Battash,
%  Amit Bleiweiss,
%  Maor Busidan,
%  Deepak R Canchi,
%  Baishali Chaudhuri,
%  Xi Chen,
%  Elad Cohen,
%  Xu Deng,
%  Pradeep Dubey,
%  Matthew Eckelman,
%  Alex Fradkin,
%  Daniel Franch,
%  Srujana Gattupalli,
%  Xiaogang Gu,
%  Amit Gur,
%  MingXiao Huang,
%  Barak Hurwitz,
%  Ramesh Jaladi,
%  Rohit Kalidindi,
%  Lior Kalman,
%  Manasa Kankanala,
%  Andrey Karpenko,
%  Noam Korem,
%  Evgeny Lazarev,
%  Hongzhen Liu,
%  Guokai Ma,
%  Andrey Malyshev,
%  Manu Prasad Manmanthan,
%  Ekaterina Matrosova,
%  Jerome Mitchell,
%  Arijit Mukhopadhyay,
%  Jitender Patil,
%  Reuven Richman,
%  Rachitha Prem Seelin,
%  Maxim Shevtshov,
%  Avi Shimalkovski,
%  Dan Shirron,
%  Hui Wu,
%  Yong Wu,
%  Ethan Xie,
%  Cong Xu,
%  Feng Yuan,
%  and
%  Eliran Zimmerman.

% \section*{MediaTek}
% Bing Yu.

% \section*{Microsoft}
% Scott McKay, Tracy Sharpe,  and
% Changming Sun.

% \section*{Myrtle}
% Peter Baldwin.

% % \textbf{Nvidia}: Po-Han Huang, Brian Pharris
% \section*{NVIDIA}

% Felix Abecassis,
%  Vikram Anjur,
%  Jeremy Appleyard,
%  Julie Bernauer,
%  Anandi Bharwani,
%  Ritika Borkar,
%  Lee Bushen,
%  Charles Chen,
%  Ethan Cheng,
%  Melissa Collins,
%  Niall Emmart,
%  Michael Fertig,
%  Prashant Gaikwad,
%  Anirban Ghosh,
%  Mitch Harwell,
%  Po-Han Huang,
%  Wenting Jiang,
%  Patrick Judd,
%  Prethvi Kashinkunti,
%  Milind Kulkarni,
%  Garvit Kulshreshta,
%  Jonas Li,
%  Allen Liu,
%  Kai Ma,
%  Alan Menezes,
%  Maxim Milakov,
%  Rick Napier,
%  Brian Nguyen,
%  Ryan Olson,
%  Robert Overman,
%  Jhalak Patel,
%  Brian Pharris,
%  Yujia Qi,
%  Randall Radmer,
%  Supriya Rao,
%  Scott Ricketts,
%  Nuno Santos,
%  Madhumita Sridhara,
%  Markus Tavenrath,
%  Rishi Thakka,
%  Ani Vaidya,
%  KS Venkatraman,
%  Jin Wang,
%  Chris Wilkerson,
%  Eric Work,
%  and
%  Bruce Zhan.

% \section*{Politecnico di Milano}
% Emanuele Vitali.

% \section*{Qualcomm}
%  Srinivasa Chaitanya Gopireddy,
%  Pradeep Jilagam,
%  Chirag Patel,
%  Harris Teague,
%  and
%  Mike Tremaine.
 
% \section*{Samsung}
% Rama Harihara,
%  Jungwook Hong,
%  David Tannenbaum,
%  Simon Waters,
%  and
%  Andy White.
 
% \section*{Stanford University}
% Peter Bailis and
% Matei Zaharia.

% \section*{Supermicro}
% Srini Bala,
%  Ravi Chintala,
%  Alec Duroy,
%  Raju Penumatcha,
%  Gayatri Pichai,
%  and
%  Sivanagaraju Yarramaneni.
 
% \section*{Unaffiliated}
% Michael Gschwind and Justin Sang.

% \section*{University of California, Berkeley / Google}
% David Patterson.

% \section*{Xilinx}
% Ziheng Gao,
%  Yiming Hu,
%  Satya Keerthi Chand Kudupudi,
%  Ji Lu,
%  Lu Tian,
%  and
%  Treeman Zheng.


 




==> tex/acks_short.tex <==
\section{Acknowledgements}
\label{sec:acks}

MLPerf Inference is the work of many individuals from numerous organizations, including the authors who led the benchmark's development and the submitters who produced the first large set of reproducible benchmark results. Both groups were necessary to create a successful industry benchmark. The list of submitters is at \url{https://arxiv.org/abs/1911.02549}. We are thankful for the feedback from anonymous reviewers and appreciate the advice and input of Cliff Young.
